Differences between Health Related News Articles from Reliable and Unreliable Media

In this study, we examine a collection of health-related news articles published by reliable and unreliable media outlets. Our analysis shows that there are structural, topical, and semantic differences in the way reliable and unreliable media outlets conduct health journalism. We argue that the findings from this study will be useful for combating health disinformation problem.

==> sec-notes.tex <==
\section{Notes}
\label{sec-notes}

\textbf{Statistics}

\url{https://tincture.io/social-life-of-health-information-a7a7aac337c}

\url{http://www.pewresearch.org/fact-tank/2014/01/15/the-social-life-of-health-information/}

% \textbf{To DO List}
% \begin{itemize}
%     \item \st{[S] Share the latest data in gitlab repository.}
%     \item \st{[S] Collect headline, author name, publish date, media links for each article using newspaper package.}
%     \item \st{[R] Apply 3 clickbait classifiers on the link-name.}
%     \item \st{[R] Check the 7 clickbait characteristics.}
%     \item \st{[R] Apply the SMS identifier on the news articles.}
%     \item \st {[S] Apply Stanford direct quote extraction.}
%     \item \st{[S] Complete the data collection phase.}
%     \item \st{[S] Write summary of the three papers and add under the Related Work} Section.
% \end{itemize}
